Structured Downsampling for Fast, Memory-efficient Curation of Online Data Streams

Operations over data streams typically hinge on efficient mechanisms to aggregate or summarize history on a rolling basis. For high-volume data steams, it is critical to manage state in a manner that is fast and memory efficient -- particularly in resource-constrained or real-time contexts. Here, we address the problem of extracting a fixed-capacity, rolling subsample from a data stream. Specifically, we explore ``data stream curation'' strategies to fulfill requirements on the composition of sample time points retained. Our ``DStream'' suite of algorithms targets three temporal coverage criteria: (1) steady coverage, where retained samples should spread evenly across elapsed data stream history; (2) stretched coverage, where early data items should be proportionally favored; and (3) tilted coverage, where recent data items should be proportionally favored. For each algorithm, we prove worst-case bounds on rolling coverage quality. We focus on the more practical, application-driven case of maximizing coverage quality given a fixed memory capacity. As a core simplifying assumption, we restrict algorithm design to a single update operation: writing from the data stream to a calculated buffer site -- with data never being read back, no metadata stored (e.g., sample timestamps), and data eviction occurring only implicitly via overwrite. Drawing only on primitive, low-level operations and ensuring full, overhead-free use of available memory, this ``DStream'' framework ideally suits domains that are resource-constrained, performance-critical, and fine-grained (e.g., individual data items as small as single bits or bytes). The proposed approach supports $\mathcal{O}(1)$ data ingestion via concise bit-level operations. To further practical applications, we provide plug-and-play open-source implementations targeting both scripted and compiled application domains.

==> Dockerfile <==
FROM mmore500/docker-texlive-full:sha-ea45eb5

COPY . /opt/hstrat-surface-concept/tex

SHELL ["/bin/bash", "-c"]

# Define default working directory.
WORKDIR /opt/hstrat-surface-concept/tex

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

# magic to fix java installation conflict in subsequent apt install
# see https://github.com/geerlingguy/ansible-role-java/issues/64
RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    man \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  mkdir /usr/share/man/man1/

RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    bibtool \
    git \
    make \
    moreutils \
    nodejs \
    pcregrep \
    pdftk \
    && \
  rm -rf /var/lib/apt/lists/*

CMD ["bash"]


==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))/..))

DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: clean all

fresher: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh fresher


==> draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> fig/doubling-instance-reservation.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/doubling-instance-reservation}
  \caption{TODO}
  \label{fig:doubling-instance-reservation}
\end{figure*}


==> fig/incrementing-instance-reservation.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/incrementing-instance-reservation}
  \caption{TODO}
  \label{fig:incrementing-instance-reservation}
\end{figure*}


==> fig/ingest-rank-calculation.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/ingest-rank-calculation}
  \caption{TODO}
  \label{fig:ingest-rank-calculation}
\end{figure*}


==> fig/instance-reservation-layout-bad.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/instance-reservation-layout-bad}
  \caption{TODO}
  \label{fig:instance-reservation-layout-bad}
\end{figure*}


==> fig/longevity-ordering.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/longevity-ordering}
  \caption{TODO}
  \label{fig:longevity-ordering}
\end{figure*}


==> fig/surface-site-ingest.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/surface-site-ingest}
  \caption{TODO}
  \label{fig:surface-site-ingest}
\end{figure*}


==> lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}

